Edisum: Summarizing and Explaining Wikipedia Edits at Scale

An edit summary is a succinct comment written by a Wikipedia editor explaining the nature of, and reasons for, an edit to a Wikipedia page. Edit summaries are crucial for maintaining the encyclopedia: they are the first thing seen by content moderators and they help them decide whether to accept or reject an edit. Additionally, edit summaries constitute a valuable data source for researchers. Unfortunately, as we show, for many edits, summaries are either missing or incomplete. To overcome this problem and help editors write useful edit summaries, we propose a model for recommending edit summaries generated by a language model trained to produce good edit summaries given the representation of an edit diff. To overcome the challenges of mixed-quality training data and efficiency requirements imposed by the scale of Wikipedia, we fine-tune a small generative language model on a curated mix of human and synthetic data. Our model performs on par with human editors. Commercial large language models are able to solve this task better than human editors, but are not well suited for Wikipedia, while open-source ones fail on this task. More broadly, we showcase how language modeling technology can be used to support humans in maintaining one of the largest and most visible projects on the Web.

==> 04_old_method.tex <==
\section{Automatic generation of Wikipedia edit summaries}
\label{sec:auto_gen_summaries}

As edit summaries serve many important purposes, both for Wikipedia and for general research, the need for automated tool that helps editors write one is clear. In \Secref{sec:qual_analysis} we show why this task is not trivial. To this day, and to our knowledge, there are no attempts to automatize this process. One of our key contributions is a first scalable solution for the task.

\subsection{Data}
\label{sec:data}

We use edits made in August 2023 to articles on English Wikipedia. This includes over 500K edits without a summary, from which we randomly take 100k edits for synthetic data generation. %which we use to generate synthetic data. From this sample, we randomly take 100K edits for synthetic data generation. 
After the initial filtering from \Secref{sec:data_collection}, we are left with around 600K edits. We additionally limit the data by filtering edits with summaries longer than 200 and shorter than 5 characters. We leave out edits from the editors who have made less than 30 edits and keep at most 3 edits with the same summary to enforce diversity. This leaves us with around 127K samples.
For experiments, we combine data obtained in both ways: from existing Wikipedia edit summaries, and by generating synthetic data. We use in total 100K samples for training, and 10K for validation. The rest is used for testing ($\sim$17K samples).

We run experiments with 5 different proportions of synthetic data in the training set (0\%, 25\%, 50\%, 75\%, 100\%), by choosing the synthetic and human editor's data randomly from the collected datasets. %For each of these datasets with mixed data, synthetic data and human editor's data samples are taken randomly from the collected datasets.
As input to the model, we use the edit diff between the two revisions of the article in question to keep the input short while preserving the most important information. We extract the difference and represent the input in the same manner as in \Secref{sec:prompt_construction}. To separate the text from the old and the new revision, we use <old\_text> and <new\_text> prefixes. Each sentence is separated by <sent\_sep> prefix. We filter out data points with inputs longer than 1,024 tokens for convenience (only 2.3\% of our data is longer than that). As the output, we use the (human- or synthetically generated) edit summary. %To represent the input, we start by concatenating all the sentences removed from the old revision into the ``old text'', and all the sentences added in the new revision into the ``new text''. Each sentence in the old/new text is separated by a <sent\_sep> prefix. Input is then formed by concatenating the old and new texts, by appending the <old\_text> and <new\_text> prefixes to the old and new texts, respectively. We filter out data points with inputs longer than 1,024 tokens for convenience, as only 2.3\% of our input data is longer than that. As the output, we use the (human- or synthetically generated) edit summary.


% \begin{itemize}
%     \item As an input to the model we use the difference between the two revisions of a Wikipedia page in question to keep the input short enough while maintaining the most important information present. It is represented as follows:
%     \begin{itemize}
%         \item We concatenate all the sentences removed from the old revision into the "old text", and all the sentences added in the new revision into the "new text".
%         \item Each sentence in the old text/new text is separated by a <sent\_sep> prefix.
%         \item Input is then formed by concatenating the old text and new, by appending <old\_text> and <new\_text> prefix to the old and new text, respectively.
%     \end{itemize}
%     \item As the output, we use the edit summary
% \end{itemize}

\subsection{Model}
Since 4.6\% of our data requires input size longer than 512 tokens used by standard small generative models \citep{chung2022scaling, lewis2019bart}, as the model to finetune, we use LongT5 \citep{guo2022longt5}, which has the ability to work with longer context windows. We denote each finetuned model as \model[$S\%$], where $S$ is a percentage of synthetic data in the training set. We intentionally use a very small model, because of limitations of Wikipedia's infrastructure. In particular, Wikipedia does not have access to many GPUs on which we could deploy big models,\footnote{\url{https://wikitech.wikimedia.org/wiki/Machine\_Learning/AMD\_GPU\#Do\_we\_have\_Nvidia\_GPUs}} meaning that we have to focus on the ones that can run on CPUs with acceptable latency. Note that this task requires a model running virtually in real-time, as edit summaries should be created when edit is performed, and cannot be precalculated to decrease the latency. Models of similar size have already been successfully implemented in Wikipedia applications. %While most of our data has input shorter than the usual 512 tokens that most of the smaller generative models work with \citep{chung2022scaling, lewis2019bart}, 4.6\% of it requires a longer context size. 
For details on implementation, see \Appref{appendix:model_implementation}.

Because this is an unexplored area, with no previous attempts to automatize the generation of Wikipedia edit summaries, there is no apparent baseline to compare against. We thus directly compare our method to the actual ground-truth data: edit summaries written by Wikipedia editors. In addition to that, we evaluate how close our model is to LLMs. We evaluate GPT-4, today's highest performing LLM from OpenAI, and GPT-3.5, which we used to generate synthetic data. We ran both LLMs on 500 randomly chosen edits from the test data. In the experiments, GPT-4 and GPT-3.5 were prompted with the same prompt used for synthetic data generation, and with the generation parameters from \Tabref{tab:generation_params}.




==> 08_future_work.tex <==
\section{Future work}
As a new language modeling task, this paper establishes what LLMs can accomplish while also demonstrating the feasibility of using much smaller language models to perform the task. Alongside these new benchmarks, this research points towards areas for improvement in future modeling efforts. For example, while we find that models trained on synthetic data outperform those trained on existing edit summaries on Wikipedia, this approach likely has limitations in learning editor community norms such as common abbreviations. We limited our training samples to edit summaries by editors with at least 30 edits based on our qualitative analysis of existing edit summaries, but future work could explore additional strategies for producing a high-quality, diverse dataset of existing edit summaries. \cite{kocetkov2022stack} found significant improvements from applying near de-duplication to their code dataset and we suspect that many edits are quite similar with minor differences and a similar pipeline might bring improvements to this task as well. The other major avenue of exploration, especially for smaller models, is how to represent an edit diff to the model. We chose a structured approach that extracted the changed sentences but this does reduce the context provided to the model, which might be beneficial for generating appropriate summaries for some edits. Future work could explore alternative approaches to determine the right balance of simplicity and efficiency to providing sufficient context for the model.

==> tables_figures/error_taxonomy.tex <==
\begin{table}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{0.19\textwidth}|p{0.16\textwidth}p{0.24\textwidth}p{0.24\textwidth}p{0.39\textwidth}p{0.24\textwidth}p{0.24\textwidth}}
\toprule
\textbf{Category} &
  Correct &
  No change &
  Not specific &
  Unclear &
  Unexhaustive &
  Unrelated \\
\midrule
\textbf{Description} &
  - &
  The summary indicates that no change was performed &
  The summary is not describing exact changes that were performed &
  The summary seems to be pointing to the correct modifications, but it is hard to understand it without looking at the diff &
  The summary does not cover all changes performed &
  The summary describes unrelated edit\\

\bottomrule
\end{tabular}%
}
\vspace{-2mm}
\caption{Taxonomy for error analysis.}
\label{tab:error_taxonomy}
\vspace{-2mm}
\end{table}

==> tables_figures/qual_analysis_taxonomy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{0.19\textwidth}|p{0.22\textwidth}p{0.24\textwidth}p{0.32\textwidth}p{0.24\textwidth}p{0.24\textwidth}p{0.24\textwidth}}
\toprule
\textbf{Criterion} &
 \textbf{Summary (what)} &
  \textbf{Summary (why)} &
  \textbf{Misleading} &
  \textbf{Inappropriate} &
  \textbf{Generate-able (what)} &
  \textbf{Generate-able (why)} \\
  \midrule
Description &
  Attempts to describe what the edit did. For example, ``added links'' &
  Attempts to describe why the edit was made. For example, ``Edited for brevity and easier reading''. &
  Overly vague or misleading per English Wikipedia guidance. For example, ``updated'' without explaining what was updated is too vague. &
  Could be perceived as inappropriate or uncivil per English Wikipedia guidance. &
  Could a language model feasibly describe the ``what'' of this edit based solely on the edit diff. &
  Could a language model feasibly describe the ``why'' of this edit based solely on the edit diff.\\
  \bottomrule
\end{tabular}%
}
\caption{Annotation criteria for qualitative analysis.}
\label{tab:annot_criteria_qual}
\end{table}

==> tables_figures/results.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.44\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/auto_res_plot.pdf}
    \vspace{-5mm}
    \caption{Results of \model\ evaluation with MoverScore. Error bars are 95\% confidence intervals (CIs). GPT-4 and GPT-3.5 perform better than \model, with the average MoverScore of 0.724 and 0.722, respectively. We do not show the performance of GPT-4 and GPT-3.5 credibly on y-axis for convenience, as their performance is susbstantially higher than for the other models. Note that both of these are shown as a dot on the plot, as there is no notion of the percentage of synthetic data in the training set for these models.}
    \label{fig:auto_results}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.54\textwidth}
        \centering
        \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{plots/aggregated_scores.pdf}
        \vspace{-2mm}
        \caption{Average aggregated scores of human evaluation. Each method was scored with 1 point for winning, 0 points for losing, and 0.5 for neither winning nor losing. Error bars are 95\% confidence intervals (CIs).}
        \label{fig:agg_scores}
        \end{subfigure}
        \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/human_eval_plot.pdf}
        \vspace{-5mm}
        \caption{Results of human evaluation. \emph{Left:} \% of time summaries from each method are chosen as the best. \emph{Right:} \% of time summaries from each method are chosen as the worst. Error bars are 95\% confidence intervals (CIs).}
        \label{fig:human_eval_results}
        \end{subfigure}
    \end{subfigure}
    \vspace{-2mm}
    \caption{Results of automatic and human evaluation.}
\vspace{-5mm}
\end{figure}
